Unbiased Bregman-Risk Estimators: Application to Regularization Parameter Selection in Tomographic Image Reconstruction

Unbiased estimators are introduced for averaged Bregman divergences which generalize Stein's Unbiased (Predictive) Risk Estimator, and the minimization of these estimators is proposed as a regularization parameter selection method for regularization of inverse problems. Numerical experiments are presented in order to show the performance of the proposed technique. Experimental results indicate a useful occurence of a concentration of measure phenomena and some implications of this hypothesis are analyzed.

==> experiment.tex <==
% \section{Application to Synchrotron $\mu$\textsc{ct} data: stripe artefacts}
% 
% In real experiments of computerized micro-tomography ($\mu$\textsc{ct}) with x-rays generated using a synchrotron,
% the data is always corrupted. The measured data is given by a function $m(\theta,t)$, which contains noise
% coming from several differents sources. Ideally, $m$ should be an image representing a stacking operator, i.e.,
% an operation that represents integration along straight lines; such an operator is called the {\it Radon transform},
% also refered as a {\it sinogram}. Since $m$ is the noisy data, it is expected that 
% $m(\theta,t) = s(\theta,t) - x(\theta,t)$ where $s$ is ideal sinogram and $x$ is a sinogram representing 
% the error. In this case, we are looking for the noise function $x$ in order to update $m$
% and have a better representation of $x$. 
% 
% One of the most typical artefacts arising in measured sinograms at synchrotron
% tomographic experiments, are the stripes on the $t$-axis. The stripes arise in the sinogram
% due to several technical reasons in the experimental setup ~\cite{miq}, as detector imperfections for instance. 
% If the stripes are not corrected, any reconstruction algorithm - taking $m$ as the input - will 
% generate ring artefacts in the final image. Several denoising algorithms were developed in 
% order to remove the stripe artefacts in the sinograms, although most depends on several 
% parameters \cite{munch,sijbers}. One of the most promising techniques is the Titarenko's method 
% \cite{tit} that depends on just one parameter of regularization.  Titarenko's approach was formulated
% in such a way that matrix $B_\gamma$ in (\ref{eq:reg_sol}) has an analytical formula. Their 
% technique was recently generalized in \cite{miq}, where a fast algorithm is presented. Titarenko's algorithm
% is refered as \textsc{ta} and it is presented here in the same context as in \cite{miq}.
% 
% We assume that the noise data $x$ does not depend on the angle, i.e., $x = x(t)$. A physical 
% motivation for this assumption is explained in \cite{tit}. In a matrix context, we are looking for 
% a vector $\vect x$ such that
% \begin{equation}
% S = M + \vect x \otimes \vect e^T, \  \ \ S,M \in \R^{R \times N}, \ \ \vect x \in \R^R, \ \vect e \in \R^N
% \end{equation}
% where $S$ and $M$ are matrices representing the two-dimensional functions $s$ and $m$, 
% respectively; $\otimes$ is the Kronecker product and $\vect e = (1,1,\ldots,1)^T$. Vector $\vect x$
% is the one that solves the ill-posed linear system $F \vect s_k = \vect 0$ for each $k=1,2,\ldots,N$, 
% where $\vect s_k$ is the $k$th column of $S$ and $F$ is a finite-difference matrix. Obviously
% we have $\vect s_k = \vect m_k + \vect x$. Therefore, vector $\vect x$  satisfies
% \begin{equation} \label{eq:hip_stripes}
% F(\vect m_k + \vect x) = \vect 0 \ \ \implica \ \ F \vect x = - F \vect m_k \ \ \implica \ \
% F \vect x = F \left( -\frac{1}{N}\sum_k \vect m_k \right)
% \end{equation}
% The noise vector $\vect x$ should be the one satisfying the ill-posed linear system
% \begin{equation} \label{eq:Fxb}
% F \vect x = \vect b, \ \ \ \vect b = - F \left( \frac{1}{N}\sum_k \vect m_k \right)
% \end{equation}
% In \cite{miq}, a Tikhonov regularization to solve (\ref{eq:Fxb}) is proposed with different
% finite-difference matrices (also called convolution matrices), exactly in the same way as 
% in (\ref{eq:tykhnov_classic}). If the first order finite-difference matrix  is used,
% \begin{equation}
% F = \left(\begin{array}{ccccccc}
% 1 & - 1 & 0 & \hdots & 0 & 0 \\
% 0 & 1 & -1 & \hdots & 0 & 0\\
% \vdots & & & \ddots & & \vdots \\
% 0 & 0 & 0 & \hdots &  - 1 & 1 
% \end{array} \right)_{R-1 \times R}
% \end{equation}
% we obtain exactly the original approach of Titarenko, where matrix $T_\gamma = (F^T F + \gamma \eye)^{-1}$
% has an explicit formula \cite{tit}. Therefore, matrix $B_\gamma = T_\gamma F^T$ in (\ref{eq:reg_sol})
% can be written analytically. 

\endinput

